Not All Relations are Equal: Mining Informative Labels for Scene Graph Generation

Scene graph generation (SGG) aims to capture a wide variety of interactions between pairs of objects, which is essential for full scene understanding. Existing SGG methods trained on the entire set of relations fail to acquire complex reasoning about visual and textual correlations due to various biases in training data. Learning on trivial relations that indicate generic spatial configuration like 'on' instead of informative relations such as 'parked on' does not enforce this complex reasoning, harming generalization. To address this problem, we propose a novel framework for SGG training that exploits relation labels based on their informativeness. Our model-agnostic training procedure imputes missing informative relations for less informative samples in the training data and trains a SGG model on the imputed labels along with existing annotations. We show that this approach can successfully be used in conjunction with state-of-the-art SGG methods and improves their performance significantly in multiple metrics on the standard Visual Genome benchmark. Furthermore, we obtain considerable improvements for unseen triplets in a more challenging zero-shot setting.

==> extra_resultsandtext.tex <==
\begin{table*}[t]
\renewcommand*{\arraystretch}{1.13}

% 	\begin{center}
		
		\resizebox{0.98\textwidth}{!}{
			\begin{tabular}{|l|c c | c  c  c  c  c  c  c  c|c  c  c  c  c  c  c  c|}
				\hline
				\multirow{3}{*}{Models} & \multicolumn{2}{c|}{Predicate Det.} &\multicolumn{8}{c|}{Phrase Det.} & \multicolumn{8}{c|}{Relationship Det.}\\
				& k =1 & calibrated k & \multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{k = 3} & \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k} &\multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{k = 3} &  \multicolumn{2}{c|}{k = 10} &\multicolumn{2}{c|}{calibrated k}  \\
				 & R@50 & R@50 & R@50  & R@100 &  R@50  & R@100  & R@50  & R@100 & R@50  & R@100 &R@50  & R@100 &  R@50  & R@100  & R@50  & R@100 & R@50  & R@100 \\
				\hline\hline 
				UVTranse[V+L] \cite{} & 55.50& 64.44 &30.11  & 36.10 & 31.93 & 40.29 & 31.85 & 40.39 & 32.46 & 40.29 & \textbf{25.74}&\textbf{29.82} & 27.39 & 34.42& 27.43& 34.60 & 27.53 & 33.10   \\ 
				LS-Net & 56.95 & 61.59 & 29.99 & 36.03 & 31.40 & 39.51 & 31.33 & 39.51 & 30.48 & 37.17 & 25.23 & 29.58 & 26.72 & 33.24 & 26.75 & 33.41& 25.58 & 30.52 \\ 
				LSV-Net & \textbf{57.61} & 64.09 & \textbf{29.94} & \textbf{36.08} & 31.75 & 40.78 & 31.51 & 40.70 & 31.12 & 39.08 & 25.28 &  29.72 & 27.04  &  34.41 & 26.96 & 34.51 & 26.15 & 32.05 \\ 
				
				\hline
				LS-Net+MutexSoftmax & 56.65 & 64.27 & 31.08 & 36.51 & 32.80 & 40.55 & 32.70 & 40.70 & 32.65 & 39.98 & 26.17 & 30.14 & 28.02 & 34.28 & 28.03 & 34.69 &  27.38 & 32.68 \\ 
				
				LSV-Net+MutexSoftmax & 56.68 & 65.99 & 30.85 & 36.59 & 32.36 & 40.35 & 32.33 & 40.19 & 33.56 & 41.66 & 25.98 & 30.03 & 27.53 & 34.08 & 27.59 & 34.22 &  27.97 & 33.78 \\
				
			    \hline
				LS-Net+MS+Implied-KL(2) & 55.90  &  68.41 & 30.03 & 35.45 & 31.51 & 39.37 & 31.32 & 38.99 & 34.24 & 42.14 & 25.26 & 29.14 & 27.08 & 33.27 & 27.00 & 33.41 &  28.44 & 34.09 \\ 
				LS-Net+MS+Implied-KL(1) &  56.26 &  63.92 & 31.08 & 36.68 & 32.77 & 40.57 & 32.74 & 40.77 & 32.12 & 39.47 & 26.33 & 30.35 & 27.93 & 34.13 & 28.00 & 34.62 &  27.17 & 32.42 \\ 
				
				\hline
				LSV-Net+MS+Implied-KL(2) & 55.51  &  69.31  & 29.05 & 34.51 & 29.85 & 38.41 & 29.16 & 37.06 & 35.70 & 43.95 & 24.64 & 28.29 & 25.67 & 32.47 & 25.24 & 31.72 &  29.44 & 35.24 \\ 
				LSV-Net+MS+Implied-KL(1) &  56.69  &  66.39 & 30.31 & 36.12 & 31.55 & 39.83 & 31.13 & 39.22 & 34.88 & 42.96 & 25.63 & 29.84 & 27.11 & 33.70 & 26.83 & 33.53 &  28.91 & 34.79 \\ 
				

				\hline \hline

				
				\rowcolor{LightCyan}
			
				\hline
			
				\rowcolor{LightCyan}
			
				\hline

\end{tabular}}
\caption{All test set performances on VRD dataset}
\label{table:alltestvrd}
\end{table*}



\begin{table*}[t]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{0.98\textwidth}{!}{
			\begin{tabular}{|l|c  >{\columncolor[gray]{0.8}}c | c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c  |c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c |}
				\hline
				\multirow{3}{*}{Models} & \multicolumn{2}{c|}{Predicate Det.} &\multicolumn{4}{c|}{Phrase Det.} & \multicolumn{4}{c|}{Relationship Det.}\\
				& k =1 & calibrated k & \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k} &  \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k}  \\
				 & R@50 & R@50 & R@50  & R@100 &  R@50  & R@100 &R@50  & R@100 &  R@50  & R@100 \\
				\hline\hline 
			
				LS-Net & 25.58 & 31.74 & 11.55 & 17.28 & 10.78 & 14.29 &10.18 & 14.88 &  8.90 &  11.04  \\ 
				LSV-Net & 27.12& 35.67 & 11.89 & 18.56 & 12.15 & 15.23 & 10.18 & 16.00 &  10.01 & 12.06  \\ 
				\hline
				LS-Net+MutexSoftmax & 26.43 & 36.78 & 13.86 & 20.19 & 14.29 & 18.14 &12.32 & 17.28 & 11.63 &  14.37  \\ 
				
				LSV-Net + MutexSoftmax & 26.86 & 38.58 & 13.34 & 19.16 & 15.57 & 19.85 & 11.98 & 17.19 &  12.40 & 15.23  \\ 
				
				\hline
				LS-Net+MS+Implied-KL (2) & 25.58 & 42.26 & 13.52 & 20.62 & 16.42 & 20.87 &11.89 & 17.62 & 13.26 &  16.42  \\ 
				
				LS-Net+MS+Implied-KL (1) & 27.20  & 35.41 & 12.75 & 20.02 & 12.23 & 16.17 &11.12 & 17.11 & 10.27 &  13.17  \\ 
				
				\hline
				LSV-Net+MS+Implied-KL (2) & 25.58 & 42.51 & 12.66 & 19.08 & 18.14 & 23.01 &11.12 & 16.17 & 14.54 &  17.79  \\ 
				
				LSV-Net+MS+Implied-KL (1) & 25.58  & 40.38 & 12.83 & 19.59 & 16.17 & 20.96 &11.04 & 17.02 & 13.00 &  16.51  \\ 
				
			       

				

				\hline
			

				\hline

\end{tabular}}
\caption{Zero Shot results on VRD dataset}
\label{table:zeroshotvrd}
\end{table*}


\begin{table*}[!tb]
\renewcommand*{\arraystretch}{1.13}

% 	\begin{center}
		
		\resizebox{0.98\textwidth}{!}{
			\begin{tabular}{|l|c >{\columncolor[gray]{0.8}}c | c  c  c  c  c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c|c  c  c  c  c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c|}
				\hline
				\multirow{3}{*}{Models} & \multicolumn{2}{c|}{Predicate Det.} &\multicolumn{8}{c|}{Phrase Det.} & \multicolumn{8}{c|}{Relationship Det.}\\
				& k =1 & calibrated k & \multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{k = 3} & \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k} &\multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{k = 3} &  \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k}  \\
				 & R@50 & R@50 & R@50  & R@100 &  R@50  & R@100  & R@50  & R@100 & R@50  & R@100 &R@50  & R@100 &  R@50  & R@100  & R@50  & R@100 & R@50  & R@100 \\
				\hline\hline 
				UVTranse[V+L] \cite{hung2020contextual} & 55.50& \textbf{64.44} &\textbf{30.11}  & \textbf{36.10} & \textbf{31.93} & 40.29 & \textbf{31.85} & 40.39 & \textbf{32.46} & \textbf{40.29} & \textbf{25.74}&\textbf{29.82} & \textbf{27.39} & \textbf{34.42} & \textbf{27.43} & \textbf{34.60} & \textbf{27.53} & \textbf{33.10}   \\ 
				LS-Net & 56.95 & 61.59 & 29.99 & 36.03 & 31.40 & 39.51 & 31.33 & 39.51 & 30.48 & 37.17 & 25.23 & 29.58 & 26.72 & 33.24 & 26.75 & 33.41& 25.58 & 30.52 \\ 
				LSV-Net & \textbf{57.61} & 64.09 & 29.94 & 36.08 & 31.75 & \textbf{40.78} & 31.51 & \textbf{40.70} & 31.12 & 39.08 & 25.28 &  29.72 & 27.04  &  34.41 & 26.96 & 34.51 & 26.15 & 32.05 \\ 
				
				\hline

			

\end{tabular}}
\caption{Comparisons of our models to UVTransE \cite{} at different values of \emph{k} and our proposed \emph{calibrated k} on the Stanford VRD dataset.}
\label{table:baselinevrd}
\end{table*}


\begin{table*}[t]
\renewcommand*{\arraystretch}{1.13}

% 	\begin{center}
		
		\resizebox{0.98\textwidth}{!}{
			\begin{tabular}{|l|c  >{\columncolor[gray]{0.8}}c | c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c  |c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c |}
				\hline
				\multirow{3}{*}{Models} & \multicolumn{2}{c|}{Predicate Det.} &\multicolumn{4}{c|}{Phrase Det.} & \multicolumn{4}{c|}{Relationship Det.}\\
				& k =1 & dynamic k & \multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{dynamic k} &  \multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{dynamic k}  \\
				 & R@50 & R@50 & R@50  & R@100 &  R@50  & R@100 &R@50  & R@100 &  R@50  & R@100 \\
				\hline\hline 
				VLK \cite{lu2016visual} & 47.87 & - & 16.17 & 17.03 & - & -  & 13.86 & 14.07 & -  & -  \\
				VTransE \cite{zhang2017visual} & 44.76 & - & 19.42 & 22.42 & - & -  & 14.07 & 15.20 & -  &  -  \\ 
				LK \cite{yu2017visual} & 55.16 & - & 23.14 & 24.03 & - &  - & 19.17 & 21.34 & -  &  - \\ 
				CAIR \cite{zhuang2017towards} & - & - & 24.04 & 25.56 & - & -  & 20.35 & 23.52 & -  & -  \\ 
				Zoom-Net \cite{yin2018zoom} & 50.69 & - & 24.82 & 28.09 & - & - & 18.92 & 21.41 & - & - \\ 
			
			    LSVR \cite{zhang2019large}  &  & - & 28.93 & 32.85 & - & -  & 23.68 & 26.67 & -  &  - \\ 
				HGAT \cite{mi2020hierarchical} & \underline{59.54} & - & - & - & - & -  & 22.52 & 24.63 & -  &-  \\ 
				RelDN \cite{zhang2019graphical} & - & - & 31.34 & 36.42 & - & -  & 25.29 & 28.62  & -  &  - \\ 
				 
				UVTransE \cite{hung2020contextual}& 55.50 & 64.44 & 30.11 & 36.10 & 32.46* & 40.29*  & 25.74 & 29.42 & 27.53*  & 35.10* \\ 
				BBCNet \cite{inayoshi2020bounding} & 57.87 & - & \underline{34.25} & \underline{40.72} & - & - & \underline{28.21} & \underline{33.36} & - & - \\ 
					\hline
				RLM-Net \cite{zhou2019visual}  &\textbf{ 57.19 }& - & \textbf{33.20} & \textbf{39.74} & - & -  & \textbf{26.55} & \textbf{31.15} & -  & - \\ 
				RLM-Net$^{\dagger}$  & 56.79 & 62.66 & 32.02 & 38.58 & 36.76 & 45.76 & 25.66 & 30.03 & 28.48 &  34.20  \\ 
				RLM-Net +Ours   & 55.87 & \textbf{66.48} & 32.00 & 38.34 & \underline{\textbf{38.29}} & \underline{\textbf{46.55}}  & 25.54 & 29.99 &  \underline{\textbf{30.01}} & \textbf{35.19}   \\ 
				
		
				\hline
				LS-Net &\textbf{ 56.95} & 61.59 & 29.99 & 36.03  & 30.48 & 37.17 & 25.23 & 29.58 & 25.58 & 30.52 \\ 
				
				LS-Net+Ours & 56.26 &\textbf{68.41}& \textbf{31.08} & \textbf{36.68} & \textbf{34.24} &  \textbf{42.14} & \textbf{26.33} & \textbf{30.35} &\textbf{28.44}  &  \textbf{34.09} \\ 
				\hline
				LSV-Net & \textbf{57.61} & 64.09 & 29.94 & 36.08 & 31.12 & 39.08 & 25.28 & 29.72 &  26.15 & 32.05 \\ 
				LSV-Net+Ours & 56.69 & \underline{\textbf{69.31}} & \textbf{30.31} & \textbf{36.12} & \textbf{35.70} & \textbf{ 43.95} & \textbf{25.63} & \textbf{29.84} & \textbf{29.44}  &  \underline{\textbf{35.24}} \\ 
			

				\hline

\end{tabular}}
\caption{Performance comparison of the Predicate, Phrase and Relationship Detection tasks on the entire VRD dataset at \emph{k=1} and our proposed \emph{calibrated k} (gray column). "-" denotes that the values are not reported or evaluated in the original papers. "*" indicates that we have re-evaluated the publicly provided model on \emph{calibrated k}. "$\dagger$" means that we have re-trained the source code available as no pre-trained models were available. The best performances in the last three blocks are marked in \textbf{bold} for comparison within that block. \underline{Underline} denotes the best performance in the whole column.\underline{\textbf{Bold}} means best performance both in the block and the whole column.}
\label{table:sota_vrd}
\end{table*}


\begin{table*}[!ht]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{0.98\textwidth}{!}{
			\begin{tabular}{|l|c  >{\columncolor[gray]{0.8}}c | c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c  |c  c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c |}
				\hline
				\multirow{3}{*}{Models} & \multicolumn{2}{c|}{Predicate Det.} &\multicolumn{4}{c|}{Phrase Det.} & \multicolumn{4}{c|}{Relationship Det.}\\
				& k =1 & calibrated k & \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k} &  \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{calibrated k}  \\
				 & R@50 & R@50 & R@50  & R@100 &  R@50  & R@100 &R@50  & R@100 &  R@50  & R@100 \\
				\hline\hline 
				VLK \cite{lu2016visual} & 8.45 & - & 3.36  & 3.75 & - & - & 3.13 & 3.52 & - & -   \\
				VTransE \cite{zhang2017visual} & - & -  & 2.65  & 3.51 & - & - &  1.71 & 2.14 & - & -   \\
				CAIR \cite{zhuang2017towards} & - & -  & 10.78  &11.30 & - & - & 9.54 & 10.26 &- & -  \\
				LK \cite{yu2017visual} & 16.98 & -  & 13.01  & 17.24 & - & - &  12.31 & 16.15 &- & -   \\
				
				
				UVTranse[V+L] \cite{hung2020contextual} & 26.49&37.04* &13.07  &18.44 & 13.43* & 17.88* &  11.00& 16.78 & 11.21*& 14.11*   \\ 
				BBCNet \cite{inayoshi2020bounding}  & \underline{27.54} & - & 12.57 & 16.51 & - & -  & 10.09 & 13.77 &   &   \\ 
				\hline
				RLM-Net \cite{zhou2019visual}  & 24.64 & - & - & - & - & -  & - & - &  - & -  \\ 
				RLM-Net$^{\dagger}$  & \textbf{25.41} & 33.19 & \textbf{8.30} & \textbf{13.00} & 11.21 & 16.85 & \textbf{7.19} & \textbf{10.69} & 8.13 &  11.55  \\ 
				RLM-Net +Ours  & 24.67 & \textbf{39.78} & 7.97 & 12.29 & \textbf{12.06} & \textbf{17.51} & 7.07 & 9.73 & \textbf{8.91} & \textbf{11.99}  \\ 
				\hline
				LS-Net & 25.58 & 31.74 & 11.55 & 17.28 & 10.78 & 14.29 &10.18 & 14.88 &  8.90 &  11.04  \\ 
				LS-Net+Ours & \textbf{25.58} &\textbf{42.26} & \underline{\textbf{13.52}} & \underline{\textbf{20.62}} & \textbf{16.42} & \textbf{20.87} & \underline{\textbf{11.89}} & \underline{\textbf{17.62}} &  \textbf{13.26} &  \textbf{16.42}  \\ 
				\hline
				LSV-Net & \textbf{27.12} & 35.67 & 11.89 & 18.56 & 12.15 & 15.23 & 10.18 & 16.00 &  10.01 & 12.06  \\ 
				LSV-Net+Ours & 25.58 & \underline{\textbf{42.51}} & \textbf{12.66} &\textbf{19.08} & \underline{\textbf{18.14}} & \underline{\textbf{23.01}} & \textbf{11.12}& \textbf{16.17} &  \underline{\textbf{14.54}} &  \underline{\textbf{17.79}}  \\
			
				\hline

\end{tabular}}
\caption{Performance on the zero-shot split of the Stanford VRD dataset. The format and definitions are the same as in \Cref{table:sota_vrd}.}
\label{table:zeroshotvrd}
\end{table*}


\begin{table}[t]
\renewcommand*{\arraystretch}{1.13}

		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c  >{\columncolor[gray]{0.8}}c | c  c c c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c  |c  c  c c  >{\columncolor[gray]{0.8}}c  >{\columncolor[gray]{0.8}}c |}
				\hline
				\multirow{3}{*}{Models} & \multicolumn{2}{c|}{Predicate Det.} &\multicolumn{6}{c|}{Phrase Det.} & \multicolumn{6}{c|}{Relationship Det.}\\
				& k =1 & calibrated k & \multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{k = 3} & \multicolumn{2}{c|}{calibrated k} &  \multicolumn{2}{c|}{k = 1} & \multicolumn{2}{c|}{k = 3} &  \multicolumn{2}{c|}{calibrated k}  \\
				 & R@50 & R@50 & R@50  & R@100 &  R@50  & R@100 &  R@50  & R@100 &R@50  & R@100 &   R@50  & R@100 &  R@50  & R@100 \\
				\hline\hline 
			
				\hline
				LSV-Net, \emph{L$_{{Softmax}_{CE}}$}  & 57.61 & 64.09 & 29.94 & 36.08 & \textbf{31.88} & \textbf{40.81} & 31.12 & 39.08 & 25.28 & 29.72 & \textbf{27.28} & 34.26 & 26.15 & 32.05 \\ 
				
				LSV-Net, \emph{L$_{BCE}$} & 57.29 & 60.63 & \textbf{30.37} & \textbf{36.61} & 31.29 & 39.68 &  30.62 & 37.77 & 25.61 & \textbf{30.26} & 26.62 & 33.33 & 25.83 & 31.21  \\ 
				
				LSV-Net, \emph{L$_{{Softmax}_{CE}}$}+\emph{L$_{KL_{imp}}$} & \textbf{57.67} & 67.48 & 27.61 & 34.17 &  29.01 & 38.39 & 30.16 & 38.65 & 23.28 & 27.82 &24.69 & 31.92 & 25.07 & 30.87  \\
				LSV-Net, \emph{L$_{{PMES}_{CE}}$}+\emph{L$_{BCE}$} & 55.98 & 65.92 & 29.58 & 35.27 & 31.04 & 39.21 & 34.37 & 42.85 & 25.03 & 29.17 & 26.70 & 33.15 & 28.61 & 34.42  \\
				LSV-Net+Ours & 56.69 & \textbf{69.31} & 30.31 & 36.12  &  31.55 & 39.83& \textbf{35.70} & \textbf{ 43.95} & \textbf{25.63} & 29.84 &27.11  &33.70 & \textbf{29.44}  &  \textbf{35.24} \\ 
			
				\hline

\end{tabular}}
\caption{Comparison of our proposed methods with other training strategies on the \emph{LSV-Net} model.}
\label{table:ablative}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rel_short.tex <==
% \noindent
% \textbf{Visual Relationship Detection}

Visual relationship detection has been extensively studied in the past few years \cite{lu2016visual, kolesnikov2019detecting, liang2018visual, bin2019mr, zhan2019exploring, zhang2017relationship, li2017vip, mi2020hierarchical, zhang2019graphical, hung2020contextual, wang2019generating, yang2018shuffle, zhang2019large, liang2019vrr, peyre2017weakly, baldassarre2020explanation}. Lu \etal \cite{lu2016visual} introduced the VRD task and dataset and proposed a combination of visual features with language priors to learn a relationship triplet. \cite{bin2019mr} and \cite{zhan2019exploring} exploit mutual relations and undetermined relationships respectively for visual relationship detection. Liang \etal \cite{liang2018visual} design a ranking based objective function to give high relevance to the annotated relationships. A limitation of their approach is that the model will fail to produce multiple plausible predicates for some pairs and overfit to the training data.
% \cite{kolesnikov2019detecting} augment the object detection pipeline with a novel box attention mechanism to model pairwise interactions between objects. 
%  Li \etal \cite{li2017vip} formulate the visual relationships triplets as a visual phrase instead of treating each entity separately.
Some related works leverage graph based formulations for message passing between objects and triplets \cite{li2018factorizable, xu2017scene, zellers2018neural,li2017scene, yin2018zoom, mi2020hierarchical}. Zhuang \etal \cite{zhuang2017towards} propose a context-aware interaction recognition framework which leads to zero-shot generalizations. 
% Zhang \etal \cite{zhang2019large} also address relationship recognition at a large scale on a version of Visual Genome dataset with 80k+ categories.
% They individually embed objects and relations into separate semantic spaces and learn correlations between them via triplet-based softmax losses.
% \cite{peyre2017weakly, baldassarre2020explanation} focus on weakly supervised learning of visual relations where the image-level annotations of subject and object are considered instead of the bounding-box instances.

To further improve relationship detection \cite{plummer2016phrase} and \cite{yu2017visual} use multiple-cues and linguistic priors from external Wikipedia data respectively. The fusion of semantic, spatial and visual features also play an important role. \textit{VTransE} \cite{zhang2017visual} and it's extension \textit{UVTransE} \cite{hung2020contextual} project different transformations of appearance features fused with language and spatial features to a predicate space. \cite{inayoshi2020bounding} combine image feature maps with semantic and spatial features before flattening them thus keeping the spatial information in the region proposals.   Zhang \etal \cite{zhang2019graphical} design graphical contrastive losses to address incorrectly paired objects in images and shows strong performance on frequently occurring relation triplets. Zhou \etal \cite{zhou2019visual} propose \emph{RLM-Net} a two-stage pipeline where first they suppress object pairs by learning relevance probabilities for pairs and then learn a graph-based predicate recognition model with multi-modal features. They cluster predicates with similar spatial positions and then smooth out the classification scores using a graph neural network. One limitation of this data driven approach is the partial label information leading to sparse and incomplete adjacency matrices, which is addressed by our manually labelled predicate correlations. For instance, in their similarity matrix the only implied label for \emph{skate on} is \emph{on}, whereas \emph{above}, \emph{ride}, \emph{stand on} are all relevant for this query predicate. 

% We benchmark their model with our proposed confidence calibration settings and also show improvements by incorporating our training strategies for smoother and more precise predicate predictions.
% To overcome this problem, \cite{xu2013speedup} exploit label correlation to propagate label information from annotated labels to missing labels.
Several methods have been proposed \cite{bucak2011multi, durand2019learning, mahajan2018exploring} for the problem of partial/missing labels in the multi-label learning setting. For image classification, in the problem of partial labels, some relevant and important labels are missing from image annotations.  However, our problem setting is slightly different from this as we deal with missing labels at the pair level and not image level. Hence, we provide novel loss formulations to incorporate label-correlations in a joint learning setting and perform remarkably well at predicting multiple and precise visual relationships. 


\begin{figure*}[!ht]
\begin{center}
\includegraphics[width=0.92\linewidth]{figures/contrib_fig.pdf}
% \vspace{-.3cm}
\end{center}
\caption{Model design of our \emph{LSV-Net} visual relationship detection model. After multi-modal feature fusion, two separate classifiers are trained with our novel loss formulations to predict predicate scores. These scores are then calibrated by our \emph{confidence calibration framework}. x and + denotes element wise product and average sum respectively.}
\label{fig:lsvmodel}
\end{figure*}


% In RLM-Net \cite{}, the authors propose a two-stage pipeline, first, they suppress object pairs by learning relevance probabilities for pairs and then learn a graph-based predicate recognition model with visual, spatial and semantic features.  


% Mutual Relation, MR-Net \cite{bin2019mr}, they explore the mutual relations between paired objects by treating the interaction between pairs in a two-way direction, \eg \emph{picture on bus} and \emph{bus has picture}. They also employ a semantic ranking loss to penalize similar predicates more mildly, for instance "next to" or "near". Although this approach has a similar motivation to ours, it is very challenging to obtain similar predicates for "implicit" relations such as walking, skating etc. Our predicate co-occurrence labelling approach bridges this gap for difficult and ambiguous visual predicates. 

% Undetermined relationships, \cite{zhan2019exploring}, They exploit the unlabelled or less relevant relationships to improve the visual relationship detection task. The multi-modal feature fusion model predicts a predicate score and a determinate confidence score to define determinate and undetermined relationships. 

% ViPCNN \cite{li2017vip}, they formulate the visual relationships triplets as a visual phrase instead of treating each entity in the triplet separately that guides the region proposals of the object detector to have more inter-dependent features. 

% Factorizable Net, \cite{li2018factorizable}, (club this with other scene graph generation methods  in a line. ) It leverages graph based message passing scheme to by using sub-graphs to facilitate visual relationship detection and scene graph generation. 

% MSDN, \cite{li2017scene}, scene graph. method, They merge the three closely related semantic tasks of object detection, region captioning and scene graph generation in an end to end manner to learn a scene description network. 

% IMP, \cite{xu2017scene}, iterative message passing 

% Neural motifs, \cite{zellers2018neural},  

% HGAT, \cite{mi2020hierarchical} constructs object-level graphs to capture interactions between objects and  triplet-level graphs to model interactions between relation triplets. This incorporates more context information in the relationship prediction task. 

% RelDN \cite{zhang2019graphical} design graphical contrastive losses to address incorrectly paired objects in images and shows strong performance on frequently occurring relation triplets in the VRD and visual genome datasets./ 


% Comprehensive image language cues, \cite{plummer2016phrase}, automatically learn weights. for combining multiple image language cues such as spatial, adjective, verb  and attribute cues for phrase localization and visual relationship detection

% Expensive feature from cheap objects, \cite{wang2019generating}, they synthesize relationship features for rare objects by randomly conditioning of different instances of the same object and show consistent improvements in zero-shot and low-shot settings. 

% Shuffle then assemble, \cite{yang2018shuffle}, proposes to generate object-agnostic features to reduce bias to frequent objects and generalize to rare or unseen objects. for doing this, they employ a cycle GAN to capture shared but not object specific information between random shuffling of object pairs. 

% RPN \cite{zhang2017relationship}, they address the problem of combinatorial explosion of forming object pairs by training a relationship proposal network that only produces meaningful pairs at test time for classifying relationships. 

% Vrr-vg, visually relevant relationships \cite{liang2019vrr} they propose a new Visually relevant relationships dataset by pruning visually irrelevant relationships and mining more relevant ones. This helps to learn more relationship specific features that improves performance on downstream tasks such as image captioning and VQA. 



% VTransE \cite{zhang2017visual}, they project the subject and object appearance features into a lower dimensional space and learn a relation translation vector to predict the predicate. This was inspired by the Translation embeddings for representing large scale knowledge bases \cite{bordes2013translating, lin2015learning}. UVTransE \cite{hung2020contextual} is an extension of the VTransE model  that projects a transformation of the union, subject and object features to the relation space which helps to learn generalized features as shown by their zero-shot performances on VRD dataset. 

% LSVRD \cite{zhang2019large}, addresses relationship recognition at a large scale on a version of Visual Genome dataset with 80k+ categories. They individually embed objects and relations into separate semantic spaces and learn correlations between them via triplet-based softmax losses. 

% Weakly supervised methods, \cite{peyre2017weakly, baldassarre2020explanation} They focus on weakly supervised learning of visual relations where the image-level annotations of subject and object are considered instead of the bounding-box instances.

% BBCNet, \cite{inayoshi2020bounding}, they fuse the image feature maps with semantic and spatial features before flattening them hence keeping the spatial information in the region proposals. 

% Zoom-Net \cite{yin2018zoom} encourage deep message interactions between local object features and global features to predict relationships. 

% InteractNet \cite{zhuang2017towards} propose a context-aware interaction recognition framework which leads to zero-shot generalizations. 

% knowledge distillation \cite{yu2017visual} They exploit linguistic priors from external Wikipedia data to improve the visual relationships using a student-teacher based distillation model. 


